AI Ethics: An Empirical Study on the Views of Practitioners and Lawmakers

Artificial Intelligence (AI) solutions and technologies are being increasingly adopted in smart systems context, however, such technologies are continuously concerned with ethical uncertainties. Various guidelines, principles, and regulatory frameworks are designed to ensure that AI technologies bring ethical well-being. However, the implications of AI ethics principles and guidelines are still being debated. To further explore the significance of AI ethics principles and relevant challenges, we conducted a survey of 99 representative AI practitioners and lawmakers (e.g., AI engineers, lawyers) from twenty countries across five continents. To the best of our knowledge, this is the first empirical study that encapsulates the perceptions of two different types of population (AI practitioners and lawmakers) and the study findings confirm that transparency, accountability, and privacy are the most critical AI ethics principles. On the other hand, lack of ethical knowledge, no legal frameworks, and lacking monitoring bodies are found the most common AI ethics challenges. The impact analysis of the challenges across AI ethics principles reveals that conflict in practice is a highly severe challenge. Moreover, the perceptions of practitioners and lawmakers are statistically correlated with significant differences for particular principles (e.g. fairness, freedom) and challenges (e.g. lacking monitoring bodies, machine distortion). Our findings stimulate further research, especially empowering existing capability maturity models to support the development and quality assessment of ethics-aware AI systems.

==> Summary_and_Implications.tex <==
\section{Key findings and implications}
We now outline the key findings of the study to answer the RQs - AI ethics principles, challenges, severity impact and the statistically significant differences between the perceptions of practitioners and lawmakers. We also report the research and practical implications of the study findings.

\subsection{Summary and interpretation of the key findings}
The results of each RQ are thoroughly discussed in Section \ref{sec:Results} and the summary of core findings is presented in Table \ref{tab:Summary of key findings}, addressing RQ1 - confirming the identified AI ethics principles and challenges, RQ2 - measuring the severity impacts of the challenges across principles and RQ3 - practitioners and lawmakers perceptions of AI ethics principles and challenges. For RQ1, the summary of the study results highlights that both practitioners and lawmakers empirically confirm the AI ethics principles and challenges identified in our recent SLR study \cite{AR13}. We noticed that ($\geq$ 60\%) of the survey participants agreed to consider the reported principles and challenges. They further define the ranks of identified principles and challenges across a five-point Likert scale, which indicates that \textit{transparency}, \textit{accountability} and \textit{privacy} are the most critical principles \cite{AR15}\cite{AR10}; on the other hand, \textit{lack of ethical knowledge}, \textit{no legal frameworks} and \textit{monitoring bodies} appeared as the most frequently occurred challenging factors. Similarly, the summary of findings to address RQ2 reveal that \textit{conflict in practice} emerged as the most severe challenging factor for the identified AI ethics principles (see Table \ref{tab:Summary of key findings}). For certain cases, the AI ethics principles come into conflict, and their practical values become unrealistic- prioritizing one might inadvertently compromise another \cite{whittlestone2019role}. Whittlestone et al. \cite{whittlestone2019role} argue that thorough exploration is required to encounter and articulate the conflict and tensions across the AI ethics principles. For RQ3, we noticed that the perceptions of both types of populations (practitioners, lawmakers) are correlated and statistically significant for specific challenges. It is because the existing principles are too vague, generic, conceptual and no match for the specific and complex AI problems. Stakeholders have different perceptions of the challenges raised because of implementing the generic AI ethics principles. A broader consensus of multiple stakeholders- practitioners, lawmakers, and regulatory bodies required to define domain-specific principles and guidelines \cite{whittlestone2019role}. Overall, the summary of the findings in Table \ref{tab:Summary of key findings} is self-explanatory and encapsulates the core results discussed in Section \ref{sec:Results}.

\begin{table*}
% \scriptsize
\centering
\caption{Summary of the key findings}
\label{tab:Summary of key findings}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{|m{3cm}|m{10cm}|}
\hline
\textbf{Research Question} & \textbf{Summary} \\ \hline
RQ1: What are the practitioners' and lawmakers' insights on AI ethics principles and challenges? & 
\begin{itemize}%[itemsep=0pt, topsep=0pt, parsep=2pt]
    \item Practitioners and lawmakers empirically confirm the principles and challenges reported in our previously published SLR study \cite{AR13}.
    \item \textit{Transparency}, \textit{accountability}, and \textit{privacy} emerged as the most perceived principles.
    \item \textit{Lack of ethical knowledge}, \textit{no legal frameworks}, and \textit{lacking monitoring bodies} appeared to be the most frequently cited challenging factors.
\end{itemize} \\
\hline
RQ2: What would be the severity impacts of identified challenges across the AI ethics principles? & 
Transparency \vspace{0mm}
\begin{itemize}%[itemsep=0pt, topsep=2pt, parsep=2pt]
    \item \textit{Interpret principles differently} has long-term impacts (50\% major, 27\% catastrophic)
    \item \textit{Lack of ethical knowledge} has short-term impacts (7\% insignificant, 25\% minor, 20\% moderate)
\end{itemize} 
Privacy \vspace{0mm}
\begin{itemize}%[itemsep=0pt, topsep=2pt, parsep=2pt]
    \item \textit{Conflict in practice} has long-term impacts (53\% major, 21\% catastrophic)
    \item \textit{Lack of technical understanding} has short-term impacts (8\% insignificant, 14\% minor, 23\% moderate)
\end{itemize} 
Accountability \vspace{0mm}
\begin{itemize}%[itemsep=0pt, topsep=2pt, parsep=2pt]
    \item \textit{Extra constraints} has long-term impacts (53\% major, 29\% catastrophic)
    \item \textit{Lack of ethical knowledge} has short-term impacts (6\% insignificant, 16\% minor, 18\% moderate)
    \item \textit{Lack of technical understanding} has short-term impacts (1\% insignificant, 18\% minor, 21\% moderate)
\end{itemize} 
Fairness \vspace{0mm}
\begin{itemize}%[itemsep=0pt, topsep=2pt, parsep=2pt]
    \item \textit{Extra constraints} has long-term impacts (49\% major, 33\% catastrophic)
    \item \textit{Interpret principles differently} has short-term impacts (3\% insignificant, 17\% minor, 24\% moderate)
\end{itemize} 
Autonomy \vspace{0mm}
\begin{itemize}%[itemsep=0pt, topsep=2pt, parsep=2pt]
    \item \textit{Conflict in practice} has long-term impacts (59\% major, 20\% catastrophic)
    \item \textit{Lack of ethical knowledge} has short-term impacts (6\% insignificant, 13\% minor, 24\% moderate)
\end{itemize} 
Explainability \vspace{0mm}
\begin{itemize}%[itemsep=0pt, topsep=2pt, parsep=2pt]
    \item \textit{Conflict in practice } has long-term impacts (55\% major, 24\% catastrophic)
    \item \textit{Lack of ethical knowledge} has short-term impacts (2\% insignificant, 12\% minor, 27\% moderate)
\end{itemize} 
\\
\hline
RQ3: How these challenges and principles are differently perceived by practitioners and lawmakers? &
\begin{itemize}%[itemsep=0pt, topsep=2pt, parsep=2pt]
    \item The perceptions of practitioners and lawmakers regarding AI ethics principles are strongly correlated (rs=0.819, p=0.000)
    \item The perceptions of practitioners and lawmakers regarding AI ethics challenges are moderately correlated (rs=0.628, p=0.012)
\end{itemize} \\
\hline
\end{tabular}%
% }
\end{table*}

\subsection{Research implications}
\begin{itemize}
    \item We found that most survey respondents agreed to consider the reported principles of AI ethics; however, \textit{transparency}, \textit{accountability} and \textit{privacy} are identified as the most common principles. The study findings complement the existing literature by revealing the most critical principles and call for future research to define the best solutions for scaling the highly significant principles in practice \cite{morley2020initial}.
    \item Regarding the challenges of AI ethics, the survey results confirm the findings of our recent SLR study \cite{AR13}, and determine \textit{lack of ethical knowledge}, \textit{no legal frameworks} and \textit{lacking monitoring bodies} as the high-ranked barriers. The identified challenges are core focus areas that need further research to explore the root causes and best practices to mitigate them.
    \item The study findings indicate that \textit{conflict in practice} is the most severe challenge of AI ethics principles. It opens the door for action-guiding future research - AI ethics principles must be contextualized to balance the conflicts \cite{whittlestone2019role}. The principles need to structure as standards, regulations and codes to resolve the conflicting tensions \cite{whittlestone2019role}.
\end{itemize}

Overall, the study findings complement the emerging research on AI ethics, particularly recognizing the perceptions of two different types of populations (practitioners and lawmakers). Researchers can quickly look up the study results and develop new hypotheses to streamline the mentioned gaps, e.g., solutions to scale the identified principles in practices, explore the causes and mitigation practices of reported challenges, and tailor the existing principles to fit in specific scenarios.
\subsection{Practical implications}
\begin{itemize}
    \item The study findings provide an overview of AI ethics principles, challenges, and practitioners can consider the overall understanding of study findings for defining ethically mature AI processes.
    \item Manifesting AI ethics principles in practice is hard because of various challenging factors. However, we measured the erroneous impacts of these challenges - revealing the most severe barriers practitioners need to tackle before embarking on ethics in AI. 
    \item In general, the study results can facilitate practitioners to get an overview and analyze the extent to which the reported principles and challenges can be leveraged to support AI ethics in the industrial setting.
 \end{itemize}
   
AI ethics in practice is still a widely unexplored research area. We invite researchers from academia and practitioners from industry to jointly contribute by sharing their experiences and to present potential solutions for AI ethics problems. This effort will bridge the gap between academia and industrial practices.  



==> Threats_to_Validity.tex <==

\section{Threats to validity}
\label{threats to validity}
Various threats could affect the validity of the study findings. We followed the guidelines presented in \cite{easterbrook2008selecting} and categorized the potential threats across the following four different types:
\subsection{Internal validity}
Internal validity refers to particular factors that impact methodological rigor. The first internal validity threat in this study is the understandability of the survey instrument. The survey participants might have a different understanding of the survey content; however, the survey instrument was piloted based on the expert's opinions to improve the readability and understandability of the questions (see Section \ref{SettingtheStage}). Moreover, the domain expertise of survey participants could be a potential internal validity threat. We tried to mitigate this threat by exploring various social media networks and used personal links to approach the most suitable candidates. Furthermore, we explicitly mentioned the characteristics of prospective participants in the survey information sheet \cite{replication}. The interpersonal bias in the data collection and analysis process could threaten the internal validity of study findings. However, the survey data is collected, analyzed, organized and reported based on the final consensus made by all the authors (see Section \ref{SettingtheStage} and Section \ref{sec:Results}). 
\subsection{Construct validity}
Construct validity is the extent to which the study constructs are well-interpreted and defended. In this study, AI ethics principles and challenges are the core constructs. The reliability and authenticity of the selected data sources (platforms) is a possible construct validity threat. This threat has been alleviated by searching social media and professional research networks to identify the most relevant groups or individuals. We thoroughly read the group discussions to ensure that the group members mainly discussed AI ethics issues. Similarly, we explored the profile details and interests of the targeted individuals. 
\subsection{External validity}
External validity is the extent to which the study findings based on a particular data sample could be broadly generalized to other contexts. The survey sample size might not be representative to provide a concrete foundation for generalizing the study findings. However, we received 99 valid responses from 20 countries across 5 continents, having a diverse range of experiences, working in various domains on distinct roles in different size organizations (see Figure \ref{Fig:Demographics}). We concede that the study findings could not be generalized at a large scale or consider the identified principles and challenges for all types of AI systems. However, considering the demographic details of the survey respondents (see Figure \ref{Fig:Demographics}), we believe that the study results can support the overall generalizability to some extent.   
\subsection{Conclusion validity}
Conclusion validity is the extent to which certain factors affect valid conclusions in empirical research. To lessen this threat, the first two authors mainly participated in the data collection process; however, the next authors participated in the consent meetings to share feedback and review the survey activities (see Section \ref{SettingtheStage}). Similarly, the third author conducted the data analysis, and the final results were presented based on the feedback shared by all the authors (see Section \ref{sec:Results}). Finally, all the authors were invited to participate in the brainstorming sessions to discuss the core findings and draw concrete conclusions. 

